A Survey on Adversarial Attacks for Malware Analysis

Machine learning has witnessed tremendous growth in its adoption and advancement in the last decade. The evolution of machine learning from traditional algorithms to modern deep learning architectures has shaped the way today's technology functions. Its unprecedented ability to discover knowledge/patterns from unstructured data and automate the decision-making process led to its application in wide domains. High flying machine learning arena has been recently pegged back by the introduction of adversarial attacks. Adversaries are able to modify data, maximizing the classification error of the models. The discovery of blind spots in machine learning models has been exploited by adversarial attackers by generating subtle intentional perturbations in test samples. Increasing dependency on data has paved the blueprint for ever-high incentives to camouflage machine learning models. To cope with probable catastrophic consequences in the future, continuous research is required to find vulnerabilities in form of adversarial and design remedies in systems. This survey aims at providing the encyclopedic introduction to adversarial attacks that are carried out against malware detection systems. The paper will introduce various machine learning techniques used to generate adversarial and explain the structure of target files. The survey will also model the threat posed by the adversary and followed by brief descriptions of widely accepted adversarial algorithms. Work will provide a taxonomy of adversarial evasion attacks on the basis of attack domain and adversarial generation techniques. Adversarial evasion attacks carried out against malware detectors will be discussed briefly under each taxonomical headings and compared with concomitant researches. Analyzing the current research challenges in an adversarial generation, the survey will conclude by pinpointing the open future research directions.

==> Farming-table-1-revised.tex <==

\begin{table*}
\centering
{
    \rowcolors{1}{lightgray!20!}{}
    \begin{tabularx}{\textwidth}{X|X|X|X}
    \hline
    \textbf{Paper Title} & 
    \textbf{Focus/Objective} & 
    \textbf{Contribution} & 
    \textbf{Limitation} &
    \hline
    %==========================================%
%    \textbf{Cyber Attacks, Threats and Proposed Solutions} &
%     &
%     &
%     &
%    \hline 
    \multicolumn{4}{l}{\textbf{\hl{Cyber Attacks, Threats and Proposed Solutions}}}\\
    \hline 
    %==========================================%
   Threats to Precision Agriculture \cite{precision_dhs} &
    \hl{Identifies} security threats, vulnerabilities, and threat scenarios in smart agriculture, crop and livestock. &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Uncovers} threats using CIA model of information security.
        \item \hl{Defines} precision agriculture technologies.
        \item \hl{Proposes} security best practices.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item Lacks distinction among threats in CPS and precision agriculture.
        \item Limited and abstract cybersecurity solutions.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
     &
    \hline 
    %==========================================%
    Cyber Risk and Security Implications in Smart Agriculture and Food System \cite{wisconsin_jahn} &
    Demonstrates the nature of modern information risk in causing ``unknown unknown'' risks. 
    
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Emphasises} the extent of cyber insurance coverage for the agriculture sector. 
        \item Discussion on the regulatory response to use of smart devices and its impact on smart farm security. 
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item Lacks clear future technological guidance for potential risks. 
        \item Incomplete arguments on future agriculture regulations and cyber insurance. 
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    \hline
    %==========================================%
    Smart Farming Cyber Security Challenges \cite{barreto2018smart} &
    \hl{Uses} empirical methodology to highlight security  issues and challenges in smart farming. &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Discusses} security challenges including agro-terrorism, social engineering, ransomware attacks, denial of service, and \hl{cyber-espionage}.
        \item \hl{Discusses} cyber risk management framework.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
      &
       \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item No \hl{implementation} and results.
        \item No use-cases to reflect how the attacks can be orchestrated.
        \item Unclear distinction of cyber threat \hl{differences} from other domains.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    
    \hline
    %==========================================%
    Enhanced Secure Device Authentication Algorithm in P2P-based Smart Farm System \cite{chae2018enhanced} &
    \hl{Enhances} P2P communications security in smart farms \hl{through a new cryptography-based solution.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Devises} a lightweight encryption and decryption method to facilitate a robust authentication solution in smart \hl{farming} P2P communications\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item It is not clear how fast and lightweight the current solution is, compared to the existing solutions\hl{.}
        \item The proposed solution has not been tested extensively in a real world scenario\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    %==========================================%
    A Prediction Model Framework for Cyber Attacks to Precision Agriculture Technologies \cite{west2018prediction} &
    \hl{Focuses} on assessing cyber-attack vulnerabilities in the technologies (e.g., sensors, transmitters and data systems) as well as in the smart farming environment\hl{.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Constructs Common Vulnerability Scoring System (CVSS)} score based on the technologies used in a smart farm with a consideration of the smart farming environmental nature\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item CVSS fails to accurately capture \hl{the} impact of connections within the entire system\hl{.}
        \item Not suitable to assess vulnerability risks to highly diverse systems \hl{that} use diverse protocols and network topologies\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    %==========================================%
%    \textbf{Blockchain Based Research} &
%     &
%     &
%     &
%    \hline 
    \multicolumn{4}{l}{\textbf{Blockchain Related Research}}\\
    \hline
    %==========================================%
   Blockchain and IoT Based Food Traceabilty System \cite{lin2018blockchain} &
    \hl{Improves} the overall food safety issues by using blockchain to ensure food traceability.
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Tracks} various aspects of the food production cycle using IoT \hl{sensors} and blockchain technology.
        \item Sensor based verification of the food production cycle proposed.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item The framework \hl{is} constructed for a general blockchain, with specific advantages provided by a particular implementation. \hl{A generic version is missing.} 
        \item Smart contracts on the blockchain \hl{are} not implemented.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    \hline
    %==========================================%
    The Rise of Blockchain Technologies in Agriculture and Food Supply Chains \cite{kamilaris2019rise} &
    \hl{Investigates} the impact of Blockchain technology in agriculture and food supply chain\hl{.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item Critically \hl{reviews} some of the ongoing \hl{blockchain-based} projects in agriculture and food supply chain\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item There exist barriers and challenges which hinder wider popularity of Blockchain-based projects among farmers and farming systems\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    %==========================================%
    \hl{Role of Internet of Things (IoT) with Blockchain Technology for the Development of Smart Farming} \cite{awanrole} &
    \hl{Develops a framework based on IoT and blockchain technology for agriculture product tracking.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Keeps track of the entire product life cycle using blockchain technology.}
        %\item \hl{Inclusion of smart contracts in the framework to automate the entire product cycle}
        \item \hl{Builds a testbed to simulate a smart farm with 120 IoT nodes and 20 blockchain producers.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        %\item \hl{Very few related work is mentioned}
        \item \hl{No comparison to other work in literature.}
        \item \hl{Certain aspects of the simulation of the proposed framework is unclear such as what workload and probability distribution have been used.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    %==========================================%
    \hl{Agriculture on the Blockchain: Sustainable Solutions for Food, Farmers, and Financing} \cite{kim2018agriculture} &
    \hl{Explores applications of blockchain beyond the typical financial use cases in agriculture.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Provides real world use cases of organizations using blockchain for agriculture.}
        \item \hl{Uses blockchain to provide food trace-ability across the entire supply chain.}
        %\item \hl{The use of smart contracts to eliminate the presence of a middleman}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{High Level discussion about the use cases with no implementation details or results.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
   %paste AI section here to revert to the previous table layout***
    \end{tabularx}
}
\caption{Projects and Research Addressing \hl{Cybersecurity} in Smart Farming}
\label{table:existing_research}
\end{table*}

\addtocounter{table}{-1}
%-------------------------------------------------------------------
\begin{table*}
\centering
{
    \rowcolors{1}{lightgray!20!}{}
    \begin{tabularx}{\textwidth}{X|X|X|X}
    \hline
    %==========================================
     %==========================================%
%    \textbf{AI and Machine Learning Assisted Work} &
%     &
%     &
%     &
%    \hline 
    %==========================================%
    \hl{A Framework for Blockchain Based Secure Smart Green House Farming} \cite{patil2017framework} &
    \hl{Provides a light-weight security framework for smart greenhouse farms based on blockchain.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Develops distributed blockchain based framework that incorporate the notion of leader elections to avoid single point of failure.}
        \item \hl{Provides threat analysis based on availability, integrity and confidentiality and their corresponding potential attacks.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{High level conceptual framework with no implementation or experiments. No related literature and no comparison to other proposed blockchain based frameworks.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    \multicolumn{4}{l}{\textbf{\hl{AI and Machine Learning Assisted Work}}}\\
    \hline   
    %==========================================%
    Design and Implementation of IoT based Smart Security and Monitoring for Connected Smart Farming \cite{shabadi975design} &
    \hl{Proposes} a threshold based decision making system which focuses on soil condition information such as temperature and humidity\hl{.} & 
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Designs and implements} a low cost IoT based security monitoring system for environmental monitoring in smart farming\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Data analysis is very limited in terms of applied methods.}%to basic threshold decision which is a basic component of any smart farming architecture
        \item \hl{Fails} to address security and privacy issues in case of tampering with any smart farming component\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    
     \hl{Security Systems for Remote Farm} \cite{abuan2014security} &
     \hl{Focuses on the application of machine learning for pattern recognition of captured CCTV videos used in farm security.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Security system for remote farms}
        \item  \hl{ Real
time monitoring and notifications in smart farming}
        \item  \hl{Image Processing and pattern recognition detected through
surveillance system of smart farms}
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{The proposed solution is not scalable}
        \item \hl{It is not clear how multiple images from several cameras can be processed and analyzed in parallel in order to satisfy the real time property of the proposed system}
        
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
     &
    \hline
    
    \hl{Edge AI in Smart Farming IoT: CNNs at the Edge and Fog Computing with LoRa} \cite{gia2019edge} &
     \hl{Expands the possibilities of smart agriculture and farming applications with Edge and Fog computing through low-power wide-area networks (LPWAN).} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item  \hl{Solves the problem of low-bandwidth transmissions with LPWANs.}
        \item  \hl{Moves data analytic and compression toward end devices to extend the functionalities of LPWANs-based smart farming systems on the edge.}
        
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Limited testbed and experiments.}
        \item \hl{The proposed system has no resiliency against saturation attacks which can be leveraged by attackers to seriously interrupt smart farming systems.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
     &
    \hline
    
    \hl{Big Data analysis for smart farming: results of TO2 project in theme food security } \cite{kempenaar2016big} &
     \hl{Uses machine learning in big data analytic for smart farming security, with a use case in milk production chain.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item  \hl{Develops a big data analytic platform for smart farming.}
        \item  \hl{Works with two different machine learning techniques.}
        
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{The proposed system has been evaluated in a very limited number of use cases and its robustness in a real world scenario is unclear.}
        
        
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
     &
    \hline
    
    %==========================================%
    \multicolumn{4}{l}{\textbf{\hl{Other Relevant Literature}}}\\
    \hline 
  
    %==========================================%
    A Framework for Cyber Security Approaches in Precision Farming \cite{chi2017framework} &
    \hl{Discusses} challenges of wireless sensor network (WSN) in digital farm, and \hl{proposes a framework of security approach for} data flow in precision agriculture\hl{.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Proposes} a  cyber physical architecture introducing the notion of virtual farms.
        \item \hl{Proposed cyber physical system offers} real time high frequency decision systems\hl{.}
        \item \hl{Discusses} security framework elements.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item High level conceptual abstract framework.
        \item No implementation prototypes or evaluation results.
        \item Incomplete data protection techniques.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
     &
    \hline
        %==========================================%
    Cyber Security in AgriFood Sector \cite{bogaardt2016cybersecurity} &
    Discusses data security challenges within the agrifood sector\hl{.} & 
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Provides} use cases showing the increase of data in the agrifood sector and their need of data security measurements\hl{.}
        \item Interviewed companies about their cybersecurity concerns\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item No security solutions. 
        \item Limited scope to data security.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    %==========================================%
    Cyber Security on the Farm: An Assessment of Cyber Security Practices in the United States Agriculture Industry \cite{geil2018cyber} & 
    \hl{Surveys} farmers and agribusiness owners about their perceptions of cybersecurity, and how age, gender, and education might affect these perceptions.
    & 
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item Quantifies levels of previous cyber-crime victimization and technology implementation.
        \item Details how individuals react to known threats, and what motivates them to adopt protection technologies.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    & \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item A temporal analysis will further add to the understanding of how cyber threat perceptions change with more awareness. 
    \end{itemize} 
    \vspace{1mm}
    \end{minipage}
    &
    \hline
    %==========================================%
    Cyberbiosecurity: A New Perspective on Protecting US Food and Agricultural System \cite{duncan2019cyberbiosecurity} &
    \hl{Defines} bio economy and \hl{investigates} cyberbioeconomy security\hl{.} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item \hl{Discusses} how current and emerging data and infrastructure security issues affect the U.S. food and agricultural system and its cybersecurity.
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item No feasible solution has been suggested to enhance cyberbioeconomy security\hl{.}
    \end{itemize} 
    \vspace{1mm}
    \end{minipage} &
    \hline
    \end{tabularx}
}
\caption{Projects and Research Addressing \hl{Cybersecurity} in Smart Farming (Continued)}
\end{table*}


